Thalamocortical contribution to solving credit assignment in neural systems

Animal brains evolved to optimize behavior in dynamically changing environments, selecting actions that maximize future rewards. A large body of experimental work indicates that such optimization changes the wiring of neural circuits, appropriately mapping environmental input onto behavioral outputs. A major unsolved scientific question is how optimal wiring adjustments, which must target the connections responsible for rewards, can be accomplished when the relation between sensory inputs, action taken, environmental context with rewards is ambiguous. The computational problem of properly targeting cues, contexts and actions that lead to reward is known as structural, contextual and temporal credit assignment respectively. In this review, we survey prior approaches to these three types of problems and advance the notion that the brain's specialized neural architectures provide efficient solutions. Within this framework, the thalamus with its cortical and basal ganglia interactions serve as a systems-level solution to credit assignment. Specifically, we propose that thalamocortical interaction is the locus of meta-learning where the thalamus provides cortical control functions that parametrize the cortical activity association space. By selecting among these control functions, the basal ganglia hierarchically guide thalamocortical plasticity across two timescales to enable meta-learning. The faster timescale establishes contextual associations to enable rapid behavioral flexibility while the slower one enables generalization to new contexts. Incorporating different thalamic control functions under this framework clarifies how thalamocortical-basal ganglia interactions may simultaneously solve the three credit assignment problems.

==> Thalamus review/garbage.tex <==

%%%%%%%%%%%
% GARBAGE %
%%%%%%%%%%%
\section{Garbage: $\sum_{i=2}^n\bw_{t,i}^2$}
We use $\Phi_t=\sum_{i=2}^n\bw_{t,i}^2$ as the potential function at time $t$. Observe that

\begin{align*}
\Exp\left[\Phi_{t+1}\ |\ \mathcal{F}_t\right] &= \Exp\left[\sum_{i=2}^n\bw_{t,i}^2+2\beta_t\Delta_{t,i}\bw_{t,i}+\beta_t^2\Delta_{t,i}^2\ |\ \mathcal{F}_t\right]\\
&\leq \Phi_t + 2\beta_t\cdot\left[\sum_{i=2}^n\left(\lambda_i-\sum_{j=1}^n\lambda_j\bw_{t,j}^2\right)\bw_{t,i}^2\right] + 4\beta_t^2\\
&= \Phi_t + 2\beta_t\cdot\left[\sum_{j=1}^n\lambda_j\bw_{t,j}^2 - \lambda_1\bw_{t,1}^2-\sum_{j=1}^n\lambda_j\bw_{t,j}^2\cdot\left(\|\bw_t\|_2^2-\bw_{t,1}^2\right)\right]+4\beta_t^2,
\intertext{By rearranging the terms, we have}
&= \Phi_t + 2\beta_t\cdot\left[\sum_{j=1}^n\lambda_j\bw_{t,j}^2\cdot\left(1-\|\bw_t\|_2^2\right)+\left(\sum_{j=1}^n\lambda_j\bw_{t,j}^2-\lambda_1\right)\cdot\bw_{t,1}^2\right] + 4\beta_t^2\\
(\because\autoref{lem:oja ub})&\leq \Phi_t + 2\beta_t\cdot\left[\gamma\cdot\sum_{j=1}^n\lambda_j\bw_{t,j}^2+\left(\sum_{j=1}^n\lambda_j\bw_{t,j}^2-\lambda_1\right)\cdot\bw_{t,1}^2\right] + 4\beta_t^2 \, .
\end{align*}
Let us zoom into the second term of the last inequality.
\begin{align*}
\gamma\cdot\sum_{j=1}^n\lambda_j\bw_{t,j}^2+\left(\sum_{j=1}^n\lambda_j\bw_{t,j}^2-\lambda_1\right)\cdot\bw_{t,1}^2 &\leq\gamma\lambda_2\Phi_t + \gamma\lambda_1\bw_{t,1}^2+\left(\lambda_2\Phi_t+\lambda_1\bw_{t,1}^2-\lambda_1\right)\cdot\bw_{t,1}^2\\
&=(1+\gamma)\lambda_2\Phi_t-(1-\gamma)\lambda_1\bw_{t,1}^2+\lambda_1(\|\bw_t\|_2^2-\Phi_t)\cdot\bw_{t,1}^2
\end{align*}




\section{Garbage: $\bw_{t,1}^2$}
\begin{theorem}\label{thm:oja w1 square weak}
For any $\epsilon,\delta\in(0,1)$, if $0\leq\beta_t\leq\min\{\frac{\epsilon\delta(\lambda_1-\lambda_2)}{16(\lambda_1+\lambda_2)},\frac{\lambda_2}{8\lambda_1(\lambda_1-\lambda_2)}\}$ for all $t\in\N$, and $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some monotonically increasing function $f$, then when $t\geq f^{-1}\left(\frac{\ln n(\lambda_1+\lambda_1)}{\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}\right)$, we have $\Pr\left[\bw_{t,1}^2<1-\epsilon\right]\leq\delta$.
\end{theorem}


\begin{table}[h]\label{table:oja w1 square weak}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
$\{\beta_t\}_{t\in\N}$                    & $f(t)$  & $f^{-1}(T)$                     & Convergence rate \\ \hline
$\beta_t=\frac{c_1}{(c_0+t)}$                     & $c_1\ln\left(\frac{t}{c_0}\right)$    & $c_0\exp(\frac{T}{c_1})$                 & $c_0\exp\left(\frac{\ln n(\lambda_1+\lambda_2)}{c_1\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}\right)$  \\ \hline
$\beta_t=c_1(c_0+t)^{\alpha-1}$, $\alpha\in(0,1)$ & $\frac{c_1}{\alpha}\left(t^{\alpha}-c_0^\alpha\right)$ &  $\left(\frac{\alpha T}{c_1}+c_0^\alpha\right)^{1/\alpha}$   & $\left(\frac{\alpha \ln n(\lambda_1+\lambda_2)}{c_1\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}+c_0^\alpha\right)^{1/\alpha}$    \\ \hline
$\beta_t=c$                               & $ct$        &       $\frac{T}{c}$          & $\frac{\ln n(\lambda_1+\lambda_2)}{c\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}$  \\ \hline
\end{tabular}
\caption{Convergence rate of Oja's rule from~\autoref{thm:oja w1 square weak} for different choices of $\{\beta_t\}_{t\in\N}$.}
\end{table}



In the following, we are going to use $\bw_{t,1}^2$ as the potential function and show that when $t$ is sufficiently large, the expectation of $\bw_{t,1}^2$ will be close to $1$. Thus, combining with~\autoref{lem:oja w norm ub}, we know that $\bw_{t,1}^2$ is close to $1$ with good probability.


For any $t\in\N$, consider the expectation of the square of the $(t+1)^{\text{th}}$ update, \textit{i.e.,} $\bw_{t+1,1}=\bw_{t,1}+\beta_t\Delta_{t,1}$, as follows.
\begin{equation}\label{eq:oja w1 square exp 1}
\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] = \bw_{t,1}^2 + 2\beta_t\cdot\left(\lambda_1-\sum_{i=1}^n\lambda_i\bw_{t,i}^2\right)\cdot\bw_{t,1}^2 + O(\beta_t^2) \, .
\end{equation}
The last term is actually within $[0,4\beta_t^2]$ due to the fact that $\Exp\left[\|\Delta_{t}\|_2^2\ |\ \mathcal{F}_t\right]\leq 4$. Now, rearrange the second term of~\autoref{eq:oja w1 square exp 1}, we have
\begin{align}
\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] &= \bw_{t,1}^2 + 2\beta_t\cdot\left[\lambda_1\bw_{t,1}^2-\lambda_1\bw_{t,1}^4 - \sum_{i=2}^n\lambda_i\bw_{t,i}^2\bw_{t,1}^2\right] + O(\beta_t^2)\nonumber\\
&\geq \bw_{t,1}^2 + 2\beta_t\cdot\left[\lambda_1\bw_{t,1}^2-\lambda_1\bw_{t,1}^4 - \lambda_2(\|\bw_t\|_2^2-\bw_{t,1}^2)\bw_{t,1}^2\right] + O(\beta_t^2)\nonumber\\
&\geq \bw_{t,1}^2 + 2\beta_t\cdot\left[\left(\lambda_1-(1+\gamma)\lambda_2\right)\bw_{t,1}^2-(\lambda_1-\lambda_2)\bw_{t,i}^4\right] + O(\beta_t^2) \, .\label{eq:oja w1 square exp 2}
\end{align}
The last inequality uses~\autoref{lem:oja w norm ub} to guarantee that $\|\bw_t\|_2^2\leq1+\gamma$.


\begin{lemma}\label{lem:oja w1 square exp}
For any $\epsilon\in(0,1)$, if $0\leq\beta_t\leq\min\{\frac{\epsilon(\lambda_1-\lambda_2)}{32\lambda_2},\frac{\lambda_2}{8\lambda_1(\lambda_1-\lambda_2)}\}$ for all $t\in\N$, and $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some monotonically increasing function $f$, then when $t\geq f^{-1}\left(\frac{2\ln n}{\epsilon(\lambda_1-\lambda_2)}\right)$, we have $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$.
\end{lemma}

\begin{proof}[Proof of~\autoref{lem:oja w1 square exp}]

\begin{claim}\label{claim:oja w1 square sink}
For any $t\in\N$ and $\epsilon\geq2\beta_t(\lambda_1-\lambda_2)(1+\gamma)^2$. If $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$, then $\Exp\left[\bw_{t+1,1}^2\right]\geq1-2\epsilon$.
\end{claim}
\begin{proof}[Proof of~\autoref{claim:oja w1 square sink}]
First, observe that $\Exp\left[\bw_{t,1}^4\right]=\Var\left[\bw_{t,1}^2\right]+\Exp\left[\bw_{t,1}^2\right]^2\geq(1-\epsilon)^2$.
Note that
\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right] &= \Exp\left[\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_{t}\right]\right]\\
(\autoref{eq:oja w1 square exp 2})&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t\cdot\left[\left(\lambda_1-(1+\gamma)\lambda_2\right)\bw_{t,1}^2-2\beta_t(\lambda_1-\lambda_2)\bw_{t,i}^4\right] + O(\beta_t^2)\right]\\
&\geq\Exp\left[\bw_{t,1}^2\right] - 2\beta_t(\lambda_1-\lambda_2)(1+\gamma)^2 \, .
\end{align*}
By the choice of $\epsilon$, $\gamma$, and $\beta_t$ (s.t. {\color{red} $\epsilon\geq2\beta_t(\lambda_1-\lambda_2)(1+\gamma)^2$}), we have $\Exp\left[\bw_{t+1,1}^2\right]\geq1-2\epsilon$.
\end{proof}

\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right] &= \Exp\left[\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_{t}\right]\right]\\
(\autoref{eq:oja w1 square exp 2})&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t\cdot\left[\left(\lambda_1-(1+\gamma)\lambda_2\right)\bw_{t,1}^2-2\beta_t(\lambda_1-\lambda_2)\bw_{t,i}^4\right]\right]\\
&=\int_{w=0}^{\sqrt{1+\gamma}}\left[\left(1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2\right)\right)\cdot w^2-(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]
\end{align*}
First,
\begin{align*}
&\int_{w=0}^{\sqrt{1-\epsilon}}\left[\left(1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2\right)\right)\cdot w^2-2\beta_t(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\\
\geq&\int_{w=0}^{\sqrt{1-\epsilon}}\left[1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2-(1-\epsilon)(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right] \\
=&\int_{w=0}^{\sqrt{1-\epsilon}}\left[1+2\beta_t\left(\frac{\epsilon}{2}(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right] \, .
\end{align*}
Next,
\begin{align}
&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[\left(1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2\right)\right)\cdot w^2-2\beta_t(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\nonumber\\
=&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2-(1-\epsilon)(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\nonumber\\
+&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}2\beta_t\left[(1-\epsilon)(\lambda_1-\lambda_2)w^2-(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\label{eq:oja w1 square int 1}
\end{align}
Suppose $\Exp\left[\bw_{t,1}^2\right]\leq\tau$, then $\Pr\left[\bw_{t,1}^2\geq1-\epsilon\right]\leq\frac{\tau}{1-\epsilon}$.
\begin{align*}
\autoref{eq:oja w1 square int 1}\geq&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2-(1-\epsilon)(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\\
+&2\beta_t\left[(1-\epsilon)(\lambda_1-\lambda_2)(1+\gamma)-(\lambda_1-\lambda_2)(1+\gamma)^2\right]\cdot\tau\\
=&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[1+2\beta_t\left(\frac{\epsilon}{2}(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\\
-&2\beta_t\tau(\lambda_1-\lambda_2)(1+\gamma)(\epsilon+\gamma) \, .
\end{align*}
Combine the two we have
\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right]&\geq \left[1+2\beta_t\left(\frac{\epsilon}{2}(\lambda_1-\lambda_2)\right)\right]\cdot \Exp\left[\bw_{t,1}^2\right] - 2\beta_t\tau(\lambda_1-\lambda_2)(1+\gamma)(\epsilon+\gamma) \, .
\end{align*}



---

Let us start with some observation on the expectation of the updates.

\vspace{2mm}
\noindent\textbf{Phase 1 ($\Exp\left[\bw_{t,1}^2\right]<1-\epsilon$).}
In this case, we are going to show that the expectation of $\bw_{t+1,1}^2$ increases by a non-negligible amount of growth.
\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right] &=\Exp\left[\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right]\right]\\
(\autoref{eq:oja w1 square exp 2})&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t(\lambda_1-(1+\gamma)\lambda_2)\bw_{t,1}^2-(\lambda_1-\lambda_2)\bw_{t,1}^4 + O(\beta_t^2)\right]\\
()&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t\left[(\lambda_1-(1+\gamma)\lambda_2)-(\lambda_1-\lambda_2)\right]\bw_{t,1}^2 + O(\beta_t^2)\right]\\
&\geq \bw_{t,1}^2 + \epsilon\beta_t(\lambda_1-\lambda_2)\bw_{t,1}^2
\end{align*}
where the last inequality is due to the choice of $\gamma$ ({\color{red} $\gamma\leq\frac{\epsilon(\lambda_1-\lambda_2)}{2\lambda_2}$}) such that $\lambda_1-(1+\gamma)\lambda_2\geq(1-\epsilon/2)(\lambda_1-\lambda_2)$.

\vspace{2mm}
\noindent\textbf{Phase 2 ($1-\epsilon\leq\bw_{t,1}^2$).}
In this case, we are going to show that the expectation of $\bw_{t+1,t}^2$ is still larger than $1-\epsilon$. Consider two cases: (i) $1-\epsilon\leq\bw_{t,1}^2\leq1-\epsilon/2$ and (ii) $1-\epsilon/2\leq\bw_{t,1}^2\leq1+\gamma$. For case (i), using the same argument in Phase 1, one can see that $\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] \geq \bw_{t,1}^2\geq1-\epsilon$.
For case (ii), we have
\begin{align}
\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] &\geq \bw_{t,1}^2 + 2\beta_t\left[(1-\epsilon/2)(\lambda_1-\lambda_2)\bw_{t,1}^2-(\lambda_1-\lambda_2)\bw_{t,1}^4\right] + O(\beta_t^2)\nonumber\\
&\geq \bw_{t,1}^2 + 2\beta_t(\lambda_1-\lambda_2)(1+\gamma)\left[(1-\epsilon/2)-(1+\gamma)\right]\nonumber\\
&\geq\bw_{t,1}^2 -2\beta_t(\lambda_1-\lambda_2)(1+\gamma)(\epsilon/2+\gamma) \, .\label{eq:oja w1 square phase 2}
\end{align}
By the choice of $\beta_t$ ({\color{red} $\beta_t\leq\frac{\epsilon}{4(\lambda_1-\lambda_2)(1+\gamma)(\epsilon/2+\gamma)}$}), the last term in the last inequality is at least $-\epsilon/2$ and thus we still have $\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] \geq \bw_{t,1}^2-\epsilon/2\geq1-\epsilon$.


Now, we are ready to show that when $t\geq f^{-1}\left(\frac{2\ln n}{\epsilon(\lambda_1-\lambda_2)}\right)$, $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$. First, let us rewrite $\Exp\left[\bw_{t,1}^2\right]$ using the filtration for $\{\bw_t\}_{t\in\N}$ as follows.
$$
\Exp\left[\bw_{t,1}^2\right] = \Exp\left[\Exp\left[\cdots\Exp\left[\bw_{t,1}^2\ |\ \mathcal{F}_{t-1}\right]\cdots\right]\ |\ \mathcal{F}_0\right] \, .
$$
For the sake of contradiction, suppose $\Exp\left[\bw_{t,1}^2\right]<1-\epsilon$. By the above discussion, for each $t'=1,2,\dots,t-1$, we have
$$
\Exp\left[\bw_{t'+1,1}^2\ |\ \mathcal{F}_{t'}\right]\geq(1+\epsilon\beta_t(\lambda_1-\lambda_2))\cdot\bw_{t',1}^2 \, .
$$
By the choice of $\beta_{t'}$ ({\color{red} $\beta_{t'}\leq\frac{1}{2\epsilon(\lambda_1-\lambda_2)}$}), we have $(1+\epsilon\beta_{t'}(\lambda_1-\lambda_2))\geq\exp(\epsilon\beta_t(\lambda_1-\lambda_2))$ for each $t'\in\N$.
Thus,
\begin{align*}
\Exp\left[\bw_{t,1}^2\right] &\geq \prod_{t'=0}^{t-1}(1+\epsilon\beta_{t'}(\lambda_1-\lambda_2))\cdot \bw_{0,1}^2\\
&\geq \exp\left(\frac{\epsilon(\lambda_1-\lambda_2)}{2}\sum_{t'=0}^{t-1}\beta_{t'}\right)\cdot\frac{1}{n}\\
&\geq1-\epsilon
\end{align*}
which is a contradiction. Thus, we conclude that $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$.
\end{proof}



\begin{proof}[Proof of~\autoref{thm:oja w1 square weak}]
Pick $\epsilon'=\frac{2\epsilon\delta\lambda_2}{\lambda_1+\lambda_2}$ and $\gamma=\frac{\epsilon'(\lambda_1-\lambda_2)}{2\lambda_2}$ such that $\frac{\epsilon'+\gamma}{\epsilon+\gamma}\leq\delta$. Apply~\autoref{lem:oja w1 square exp} using $\epsilon'$, when $t\geq f^{-1}\left(\frac{\ln n(\lambda_1+\lambda_1)}{\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}\right)=f^{-1}\left(\frac{2\ln n}{\epsilon'(\lambda_1-\lambda_2)}\right)$, we have $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon'$. Next, by~\autoref{lem:oja w norm ub}, we can upper bound the expectation as follows. Let $p=\Pr\left[\bw_{t,1}^2<1-\epsilon\right]$, we have
$$
\Exp\left[\bw_{t,1}^2\right]\leq (1-\epsilon)p+(1+\gamma)(1-p) = 1+\gamma-(\epsilon+\gamma)p
$$
and thus
$$
p\leq\frac{\epsilon'+\gamma}{\epsilon+\gamma}\leq\delta.
$$
\end{proof}



%%%%%%%%%%%
% Garbage %
%%%%%%%%%%%
\section{Garbage: Log ratio}
\begin{theorem}\label{thm:oja Chebyshev}
For any $\epsilon,\delta\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some function $f$ where $\lim_{t\rightarrow\infty}f(t)=\infty$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then when $t\geq \max\{f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{\lambda_1-\lambda_2}\right),f^{-1}\left(\frac{\sqrt{O(1)/\delta}+\frac{1}{2}\ln n+O(1)}{\lambda_1-\lambda_2}\right)\}$, with probability $1-\delta$, we have
$$
\frac{\bw_{t,1}^2}{\|\bw_t\|_2^2}\geq1-\epsilon \, .
$$
\end{theorem}

\iffalse
\begin{theorem}\label{thm:oja Chebyshev}
For any $\epsilon,\delta\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq\alpha\cdot\ln t$ for large enough $t$ and some $\alpha>0$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then when $t\geq e^{\max\{\frac{\ln(n/\epsilon^2)+O(1)}{\alpha(\lambda_1-\lambda_2)},O(\frac{\ln(n)}{\sqrt{\delta}\alpha(\lambda_1-\lambda_2)})\}}$, with probability $1-\delta$, we have
$$
\frac{\bw_{t,1}^2}{\|\bw_t\|_2^2}\geq1-\epsilon \, .
$$
\end{theorem}
\fi

Here we state~\autoref{thm:oja Chebyshev} in a very general form with the flexibility to choose different $\{\beta_t\}_{t\in\N}$. A standard choice would be $\beta_t=\frac{c}{t}$ for some constant $c>0$ and the corresponding $f$ would be $f(t)\geq c\ln t$. In~\autoref{table:oja Chebyshev}, we list the convergence rate bounds for different choices of $\{\beta_t\}_{t\in\N}$.

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline
$\{\beta_t\}_{t\in\N}$                      & $f(t)$                       & Convergence rate                                                                                                                                                            \\ \hline
$\beta_t=\frac{c}{t}$                       & $c\ln t$                     & $t\geq\max\{ e^{\frac{\ln(n/\epsilon^2)+O(1)}{c(\lambda_1-\lambda_2)}},e^{O(\frac{\ln(n)}{\sqrt{\delta}c(\lambda_1-\lambda_2)})}\}$                                             \\ \hline
$\beta_t=ct^{\alpha-1}$, $\alpha\in(0,0.5)$ & $\frac{c}{\alpha}t^{\alpha}$ & $t\geq \max\{\left(\frac{\alpha\left(\ln(1/\epsilon)+O(1)\right)}{c(\lambda_1-\lambda_2)}\right)^{1/\alpha},\left(\frac{\alpha\left(\sqrt{O(1)/\delta}+\frac{1}{2}\ln n+O(1)\right)}{c\left(\lambda_1-\lambda_2\right)}\right)^{1/\alpha}\}$ \\ \hline
\end{tabular}
\caption{Convergence rate for different choices of $\{\beta_t\}_{t\in\N}$.}
\label{table:oja Chebyshev}
\end{table}

The proof of~\autoref{thm:oja Chebyshev} is based on the following three lemmas and Chebyshev's inequality. The first lemma shows that by properly picking $\{\beta_t\}_t$, the $\ell_2$ norm of $\bw_t$ is always close to $1$.
\begin{lemma}\label{lem:oja ub}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{\epsilon}{16}$ for all $t\in\N$, then $1-\epsilon\leq\|\bw_t\|_2^2\leq 1+\epsilon$ for all $t\in\N$.
\end{lemma}
\begin{proof}
Here we only prove the upper bound while the lower bound can be proved using the same argument.
The proof is using induction. For $t=0$, we have $\|\bw_0\|_2=1$ from the setting. For each $t\geq0$, we have
\begin{align*}
\|\bw_t+1\|_2^2 &= \|\bw_t\|_2^2 + 2\beta_t\cdot\bw_t^\top\left[\bx_t^\top\bw_t\bx_t-(\bx_t^\top\bw_t)^2\bw_t\right] + \beta_t^2\cdot\|\bx_t^\top\bw_t\bx_t-(\bx_t^\top\bw_t)^2\bw_t\|^2\\
&=\|\bw_t\|_2^2 - 2\beta_t(\bx_t^\top\bw_t)^2\cdot(\|\bw_t\|_2^2-1) + 4\beta_t^2(\bx_t^\top\bw_t)^2\cdot\max\{\|\bx_t\|_2^2,(\bx_t^\top\bw_t)^2\|\bw_t\|_2^2\} \, .
\end{align*}
Finally, consider two cases: (i) $\|\bw_t\|_2^2\leq1+\epsilon/2$ and (ii) $1+\epsilon/2<\|\bw_t\|_2^2\leq1+\epsilon$. It is then not difficult to see that by our choice of $\beta_t$, we have $\|\bw_{t+1}\|_2^2\leq1+\epsilon$ in both cases. This completes the induction and the proof.
\end{proof}

Note that~\autoref{lem:oja ub} does not depend on the structure of $A$ and holds with probability $1$.

The other two lemmas describe the expectation and the variance of the log of the ration between the $\ell_2$ mass of the first coordinate and that of the rest. However, it turns out that directly working on the log of the ratio would not work due to the unbounded second moment. As a fix, we are going to work on the \textit{truncated} version of the log ratio and show that the original log ratio behaves the same as its truncated counterpart in most of the time. To formalize the above idea, we are going to use the language from martingale theory. See~\autoref{sec:prelim} for basic definitions of martingale. 

Fix $t\in\N$ and for each $t'\in\{0,1,\dots,t\}$, let
$$
M_{t'} = \Exp\left[\sum_{i=2}^n\bw_{t,i}^2\Big|\mathcal{F}_{t'}\right] \, .
$$
It is not difficult to check that $\{M_{t'}\}_{t'\in\{0,1,\dots,t\}}$ is a martingale.
Also, observe that $M_0=\Exp\left[\sum_{i=2}^n\bw_{t,i}^2\right]$ and $M_t=\sum_{i=2}^n\bw_{t,i}^2$. Namely, $|M_t-M_0|$ is exactly the deviation of the $\ell_2$ mass to its expectation.



The second key lemma upper bounds the log of the ratio between the $\ell_2$ mass of the first coordinate and that of the rest.
\begin{lemma}\label{lem:oja ratio}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some function $f$ where $\lim_{t\rightarrow\infty}f(t)=\infty$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq\ln\left(\frac{1}{\epsilon}\cdot\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)$ when $t\geq f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{2(\lambda_1-\lambda_2)}\right)$.
\end{lemma}

\iffalse
\begin{lemma}\label{lem:oja ratio}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq\alpha\cdot\ln t$ for large enough $t$ and some $\alpha>0$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq\ln\left(\frac{1}{\epsilon}\cdot\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)$ when $t\geq e^{\frac{\ln(1/\epsilon)+O(1)}{\alpha(\lambda_1-\lambda_2)}}$.
\end{lemma}
\fi

Finally, we need the following lemma upper bounding the variance of the log ratio.
\begin{lemma}\label{lem:oja ratio variance}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$ and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $\Var\left[\sum_{i=2}^n\bw_{t,i}^2\right]=O(1)$ for all $t\in\N$.
\end{lemma}

Before we prove~\autoref{lem:oja ratio} and~\autoref{lem:oja ratio variance}, let us see how the above lemmas combining with Chebyshev's inequality imply the main theorem.
\begin{proof}[Proof of~\autoref{thm:oja Chebyshev}]
By Chebyshev's inequality, we have
$$
\Pr\left[\left|\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)-\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\right|>\sqrt{\frac{\Var[X_t]}{\delta}}\right]\leq\delta \, .
$$
Next, recall that $\bw_{0,i}^2=\frac{1}{n}$ for each $i\in[n]$ and thus by the choice of $t\geq \max\{f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{\lambda_1-\lambda_2}\right),f^{-1}\left(\frac{\sqrt{O(1)/\delta}+\frac{1}{2}\ln n+O(1)}{\lambda_1-\lambda_2}\right)\}$, \autoref{lem:oja ratio} and~\autoref{lem:oja ratio variance} give us that
$$
\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq2\ln\left(\frac{1}{\epsilon}\right),\ 2\sqrt{\frac{\Var[X_t]}{\delta}}
$$
Finally,
$$
\Pr\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)<\ln\left(\frac{1}{\epsilon}\right)\right]\leq\delta \, .
$$
\end{proof}

\subsection{Details of the expectation bound}
\begin{proof}[Proof of~\autoref{lem:oja ratio}]
Note that one can expand the expectation $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]$ using the filtration of the process $\bw_t$. Concretely, we have
\begin{equation}\label{eq:oja exp filtration}
\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right] = \Exp\left[\Exp\left[\cdots\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\Big|\ \bw_{t-1}\right]\cdots\right]\Big|\ \bw_{1}\right] \, .
\end{equation}
Now, it suffices to prove the following claim.
\begin{claim}\label{claim:oja ratio induction step}
For any $t\in\N$, we have
$$
\Exp\left[\ln\left(\bw_{t,1}^2\right)\Big|\ \bw_{t-1}\right]=\ln\left(\bw_{t-1,1}^2\right) + 2\beta_{t-1}\cdot\left(\lambda_1-\sum_{i'\in[n]}\lambda_i\bw_{t-1,i'}^2\right) + \Theta(\beta_{t-1}^2)
$$
and
$$
\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\Big|\ \bw_{t-1}\right]=\ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + 2\beta_{t-1}\cdot\left(\frac{\sum_{i=2}^n\lambda_i\bw_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right) + \Theta(\beta_{t-1}^2) \, .
$$
\end{claim}
\begin{proof}[Proof of~\autoref{claim:oja ratio induction step}]
For brevity, here we only prove the second equation while the first equation can be proved in similar argument.
By~\autoref{eq:oja}, let $\Delta_{t-1,t}=\left(y_t(\bx_t-y_t\bw_t)\right)_i$, we have
\begin{align*}
\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\Big|\ \bw_{t-1}\right] &=\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t-1,i}^2 + 2\beta_{t-1}\Delta_{t-1,i}\bw_{t-1,i} + \beta_{t-1}^2\Delta_{t-1,i}^2\right)\Big|\ \bw_{t-1}\right]\\
&= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + \Exp\left[\ln\left(1+2\beta_{t-1}\frac{\sum_{i=2}^n\Delta_{t-1,i}\bw_{t-1,i}}{\sum_{i=2}^n\bw_{t-1,i}^2} + \beta_{t-1}^2\frac{\sum_{i=2}^n\Delta_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}\right)\Big|\ \bw_{t-1}\right]\\
&= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + \Exp\left[2\beta_{t-1}\frac{\sum_{i=2}^n\Delta_{t-1,i}\bw_{t-1,i}}{\sum_{i=2}^n\bw_{t-1,i}^2} + \Theta\left(\beta_{t-1}^2\frac{\sum_{i=2}^n\Delta_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}\right)\Big|\ \bw_{t-1}\right]
\end{align*}
By~\autoref{eq:oja exp}, for each $i\in[n]$, we have 
$$
\Exp\left[\Delta_{t-1,i}\Big|\ \bw_{t-1}\right]=\left(\lambda_i-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right)\bw_{t-1,i}
$$
and thus combining with~\autoref{lem:oja ub}, we have\todo{Here I'm a bit sloppy about the $\beta_{t-1}^2$ term}
\begin{align*}
\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\Big|\ \bw_{t-1}\right] &= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + 2\beta_{t-1}\cdot\frac{\sum_{i=2}^n\left(\lambda_i-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right)\cdot\bw_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2} + \Theta(\beta_{t-1}^2)\\
&= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + 2\beta_{t-1}\cdot\left(\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right) + \Theta(\beta_{t-1}^2) \, .
\end{align*}
\end{proof}
By applying~\autoref{claim:oja ratio induction step} on~\autoref{eq:oja exp filtration}, we have
\begin{align*}
\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right] &= \Exp\left[\ln\left(\bw_{t,1}^2\right)\right] - \Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\right]\\
&=\ln\left(\bw_{0,1}^2\right) - \ln\left(\sum_{i=2}^n\bw_{0,i}^2\right)+2\sum_{t'=0}^{t-1}\beta_{t'}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) + \Theta\left(\sum_{t'=0}^{t-1}\beta_{t'}^2\right)\\
&\geq\ln\left(\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)+2(\lambda_1-\lambda_2)\cdot f(t) - O(1)\, .
\end{align*}
Note that the last inequality is due to the choice of $\{\beta_t\}_t$ where $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$.
Finally, by our choice of $t\geq f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{2(\lambda_1-\lambda_2)}\right)$, we conclude that $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq\ln\left(\frac{1}{\epsilon}\cdot\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)$.
\end{proof}

\subsection{Details of the variance bound}
\todo{Maybe need some prelim for conditional variance and filtration.}

Now, we are ready to prove~\autoref{lem:oja ratio variance} with the aid of~\autoref{lem:var decomp}.

\begin{proof}[Proof of~\autoref{lem:oja ratio variance}]
For each $t\in\N$, let $X_t=\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)$ and apply~\autoref{lem:var decomp}. The key step of the proof is showing that each summand in the variance decomposition is nicely upper bounded.
\begin{claim}\label{claim:oja ratio variance bound}
For each $t'\in\N$, we have
$$
\Exp\left[\Var\left[\Exp\left[X_t|\mathcal{F}_{t'+1}\right]|\mathcal{F}_{t'}\right]\right] = O(\beta_{t'}^2) \, .
$$
\end{claim}
Note that as $\sum_{t'=0}^\infty\beta_{t'}=O(1)$,~\autoref{claim:oja ratio variance bound} combining with~\autoref{lem:var decomp} immediately give that $\Var\left[X_t\right]=O(1)$. Now, the only thing left is proving~\autoref{claim:oja ratio variance bound}.
\begin{proof}[Proof of~\autoref{claim:oja ratio variance bound}]
Recall that from the definition of conditional variance we have
$$
\Var\left[\Exp\left[X_t|\mathcal{F}_{t'+1}\right]|\mathcal{F}_{t'}\right] = \Exp\left[\left(\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right]\right)^2\right] \, .
$$
By~\autoref{claim:oja ratio induction step}, we have
\begin{align}
\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right] &= \ln\left(\frac{\bw_{t'+1,1}^2}{\sum_{i=2}^n\bw_{t'+1,i}^2}\right) + 2\sum_{t''=t'+1}^{t-1}\beta_{t''}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t'',i}^2}{\sum_{i=2}^n\bw_{t'',i}^2}\right) + \Theta(\beta_{t''}^2)\nonumber\\
&- \left(\ln\left(\frac{\bw_{t',1}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) + 2\sum_{t''=t'}^{t-1}\beta_{t''}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t'',i}^2}{\sum_{i=2}^n\bw_{t'',i}^2}\right) + \Theta(\beta_{t''}^2)\right)\nonumber\\
&= \ln\left(\frac{\bw_{t'+1,1}^2}{\sum_{i=2}^n\bw_{t'+1,i}^2}\right) - \ln\left(\frac{\bw_{t',1}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) - 2\beta_{t'}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) + \Theta(\beta_{t'}^2) \, .\label{eq:oja ratio variance 1}
\end{align}
Recall that $\bw_{t'+1,i}=\bw_{t',i}+\beta_{t'}\cdot\Delta_{t',i}$, thus we have\todo{I'm a bit fast here, can slow down if needed.}
\begin{align}
\ln\left(\frac{\bw_{t'+1,1}^2}{\sum_{i=2}^n\bw_{t'+1,i}^2}\right) - \ln\left(\frac{\bw_{t',1}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) &= 2\beta_{t'}\cdot\left(\frac{\Delta_{t',1}}{\bw_{t',1}}-\frac{\sum_{i=2}^n\Delta_{t',i}\bw_{t',i}}{\sum_{i=2}^n\bw_{t',i}^2}\right) + \Theta(\beta_{t'}^2) \, .\label{eq:oja ratio variacne 2}
\end{align}
Combining~\autoref{eq:oja ratio variance 1} and~\autoref{eq:oja ratio variacne 2} we have
\begin{align}
\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right] &=2\beta_{t-'}\cdot\left[\left(\frac{\Delta_{t',1}}{\bw_{t',1}}-\frac{\sum_{i=2}^n\Delta_{t',i}\bw_{t',i}}{\sum_{i=2}^n\bw_{t',i}^2}\right)-\left(\lambda_1-\frac{\sum_{i=2}^2\lambda_i\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right)\right] + \Theta(\beta_{t'}^2) \, .\label{eq:oja ratio variance 3}
\end{align}
Thus, combining with~\autoref{lem:oja ub} we have\todo{I'm a bit sloppy here. Basically we still need to argue that the expectation of the square of $\frac{\Delta_{t',1}}{\bw_{t',1}}$ is $O(1)$.}
$$
\Var\left[\Exp\left[X_t|\mathcal{F}_{t'+1}\right]|\mathcal{F}_{t'}\right] = \Exp\left[\left(\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right]\right)^2\right] =O(\beta_{t'}^2)\, .
$$
\end{proof}
This completes the proof of~\autoref{lem:oja ratio variance}.
\end{proof}

\subsection{High probability bound}

To get high probability bound, \textit{i.e.,} having exponentially better dependency on error probability $\delta$, we are going to apply tools from martingale theory. Also, it is important to identify the right martingale to analyze the following is our choice. Fix $t\in\N$ and for each $t'\in\{0,1,\dots,t\}$, let
$$
M_{t'} = \Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\Big|\mathcal{F}_{t'}\right] \, .
$$
It is not difficult to check that $\{M_{t'}\}_{t'\in\{0,1,\dots,t\}}$ is a martingale.
Also, observe that $M_0=\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]$ and $M_t=\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)$. Namely, $|M_t-M_0|$ is exactly the deviation of the log ratio to its expectation. Finally, to apply concentration inequality for martingale (\textit{e.g.,} Azuma's inequality in~\autoref{lem:azuma}), it suffices to upper bound the absolute difference between $|M_{t'+1}-M_{t'}|$ for each $t'\in\{0,1,\dots,t-1\}$.

\begin{lemma}\label{lem:oja abs diff}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq\alpha\cdot\ln t$ for large enough $t$ and some $\alpha>0$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $|M_{t'+1}-M_{t'}|=O(\beta_{t'})$ with probability $1$ for each $t'\in\{0,1,\dots,t-1\}$.
\end{lemma}
\begin{proof}[Proof of~\autoref{lem:oja abs diff}]
Note that using the notation from the previous lemmas, $M_{t'}=\Exp\left[X_t|\mathcal{F}_{t'}\right]$. Thus, by~\autoref{eq:oja ratio variance 3}, we have
\begin{align*}
M_{t'+1}-M_{t'} &= \Exp\left[X_t|\mathcal{F}_{t'+1}\right] - \Exp\left[X_t|\mathcal{F}_{t'}\right]\\
&= 2\beta_{t'}\cdot\left[\left(\frac{\Delta_{t',1}}{\bw_{t',1}}-\frac{\sum_{i=2}^n\Delta_{t',i}\bw_{t',i}}{\sum_{i=2}^n\bw_{t',i}^2}\right)-\left(\lambda_1-\frac{\sum_{i=2}^2\lambda_i\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right)\right] + \Theta(\beta_{t'}^2)
\end{align*}
\end{proof}



==> Thalamus review/macros.tex <==
\newcommand{\N}{\mathbb{N}}
\newcommand{\Nz}{\mathbb{N}_{\geq0}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Var}{\mathsf{Var}}

\renewcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\bP}{\mathbb{P}}



\newcommand{\gap}{\textsf{gap}}
\newcommand{\diag}{\textsf{diag}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bbw}{\overline{\mathbf{w}}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother

\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\bigcupdot}{\charfusion[\mathop]{\bigcup}{\cdot}}

\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\veps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}

\renewcommand{\qedsymbol}{\hfill{\Large $\square$}}


% Operators
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\grad}{\nabla}
\newcommand{\hess}{\nabla^2}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\fracpar}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\iprod}[2]{\langle #1, #2 \rangle}


\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\fnorm}[1]{\left\|{#1}\right\|_{\text{F}}}
\newcommand{\spnorm}[2]{\left\| {#1} \right\|_{\text{S}({#2})}}
\newcommand{\sigmin}{\sigma_{\min}}
\newcommand{\tr}{\mathrm{tr}}
\renewcommand{\det}{\mathrm{det}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\logdet}{\mathrm{logdet}}
\newcommand{\trans}{^{\top}}
\newcommand{\proj}{\mathcal{P}}
\newcommand{\projII}{\mathcal{P}_{\parallel}}
\newcommand{\projT}{\mathcal{P}_{\perp}}

% Big O
\newcommand{\cO}{\mathcal{O}}
\newcommand{\tlO}{\mathcal{\tilde{O}}}
\newcommand{\tlOmega}{\tilde{\Omega}}


% Set
\newcommand{\Z}{\mathbb{Z}}

\renewcommand{\P}{\mathbb{P}}
\newcommand{\hP}{\hat{\mathbb{P}}}


\newcommand{\cD}{\mathcal{D}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
% Matrix and Vectors
\newcommand{\B}{\mat{B}}
\newcommand{\Q}{\mat{Q}}
\newcommand{\I}{\mat{I}}

\newcommand{\U}{\mat{U}}
\newcommand{\V}{\mat{V}}

\newcommand{\X}{\mat{X}}
\newcommand{\Y}{\mat{Y}}
\newcommand{\mSigma}{\mat{\Sigma}}
\newcommand{\mLambda}{\mat{\Lambda}}
\newcommand{\e}{\vect{e}}
\renewcommand{\u}{\vect{u}}
\renewcommand{\v}{\vect{v}}
\newcommand{\w}{\vect{w}}
\newcommand{\x}{\vect{x}}
\newcommand{\y}{\vect{y}}
\newcommand{\z}{\vect{z}}
\newcommand{\q}{\vect{q}}

\renewcommand{\L}{\mathcal{L}}
\renewcommand{\H}{\mathcal{H}}

\newcommand{\cn}{\kappa}
\newcommand{\nn}{\nonumber}


\newcommand{\ud}{{\mathrm{d}}}



\newcommand{\ind}[3]{{#1}^{#2}_{#3}} % V^k_h
\newcommand{\sind}[3]{{#1}^{#2}_{#3}} % special for V^\star_h, V^\pi_h
\newcommand{\empP}[2]{\hat{\mathbb{P}}^{#1}_{#2}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\empVV}[2]{\hat{\mathbb{V}}^{#1}_{#2}}
\newcommand{\logt}{\iota}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\Ea}{\E_{a^\star}}
\newcommand{\Pa}{\P_{a^\star}}
\newcommand{\done}{\mathbb{I}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bmu}{\bm{\mu}}

\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
% \newcommand{\M}{\mat{M}}
% \newcommand\Mmh{\mat{M}^{-1/2}}
% \newcommand{\A}{\mat{A}}
% \newcommand{\B}{\mat{B}}
% \newcommand{\C}{\mat{C}}
% \newcommand{\Et}[1][t]{\mat{E_{#1}}}
% \newcommand{\Etp}{\Et[t+1]}
% \newcommand{\Errt}[1][t]{\mat{\bigtriangleup_{#1}}}
% \newcommand\cnM{\kappa}
% \newcommand{\cn}[1]{\kappa\left(#1\right)}
% \newcommand\X{\mat{X}}
% \newcommand\fstar{f_*}
% \newcommand\Xt[1][t]{\mat{X_{#1}}}
% \newcommand\ut[1][t]{{u_{#1}}}
% \newcommand\Xtinv{\inv{\Xt}}
% \newcommand\Xtp{\mat{X_{t+1}}}
% \newcommand\Xtpinv{\inv{\left(\mat{X_{t+1}}\right)}}
% \newcommand\U{\mat{U}}
% \newcommand\UTr{\trans{\mat{U}}}
% \newcommand{\Ut}[1][t]{\mat{U_{#1}}}
% \newcommand{\Utinv}{\inv{\Ut}}
% \newcommand{\UtTr}[1][t]{\trans{\mat{U_{#1}}}}
% \newcommand\Utp{\mat{U_{t+1}}}
% \newcommand\UtpTr{\trans{\mat{U}_{t+1}}}
% \newcommand\Utptild{\mat{\widetilde{U}_{t+1}}}
% \newcommand\Us{\mat{U^\star}}
% \newcommand\UsTr{\trans{\mat{U^\star}}}
% \newcommand{\Sigs}{\mat{\Sigma}}
% \newcommand{\Sigsmh}{\Sigs^{-1/2}}
% \newcommand{\eye}{\mat{I}}
% \newcommand{\twonormbound}{\left(4+\DPhi{\M}{\Xt[0]}\right)\twonorm{\M}}
% \newcommand{\lamj}{\lambda_j}

% \renewcommand\u{\vect{u}}
% \newcommand\uTr{\trans{\vect{u}}}
% \renewcommand\v{\vect{v}}
% \newcommand\vTr{\trans{\vect{v}}}
% \newcommand\w{\vect{w}}
% \newcommand\wTr{\trans{\vect{w}}}
% \newcommand\wperp{\vect{w}_{\perp}}
% \newcommand\wperpTr{\trans{\vect{w}_{\perp}}}
% \newcommand\wj{\vect{w_j}}
% \newcommand\vj{\vect{v_j}}
% \newcommand\wjTr{\trans{\vect{w_j}}}
% \newcommand\vjTr{\trans{\vect{v_j}}}

% \newcommand{\DPhi}[2]{\ensuremath{D_{\Phi}\left(#1,#2\right)}}
% \newcommand\matmult{{\omega}}


==> Thalamus review/thmmacros.tex <==
\usepackage{amsthm}
\usepackage{thmtools,thm-restate}

\numberwithin{equation}{section}
\declaretheoremstyle[bodyfont=\it,qed=\qedsymbol]{noproofstyle} 

\declaretheorem[numberlike=equation]{axiom}

\declaretheorem[numberlike=equation]{observation}
\declaretheorem[numberlike=equation,style=noproofstyle,name=Observation]{observationwp}
\declaretheorem[name=Observation,numbered=no]{observation*}

\declaretheorem[numberlike=equation]{fact}
\declaretheorem[numberlike=equation]{subclaim}
\declaretheorem[numberlike=equation]{problem}

\declaretheorem[numberlike=equation]{theorem}
\declaretheorem[numberlike=equation,style=noproofstyle,name=Theorem]{theoremwp}
\declaretheorem[name=Theorem,numbered=no]{theorem*}

\declaretheorem[numberlike=equation]{lemma}
\declaretheorem[name=Lemma,numbered=no]{lemma*}
\declaretheorem[numberlike=equation,style=noproofstyle,name=Lemma]{lemmawp}

\declaretheorem[numberlike=equation]{corollary}
\declaretheorem[name=Corollary,numbered=no]{corollary*}
\declaretheorem[numberlike=equation,style=noproofstyle,name=Corollary]{corollarywp}

\declaretheorem[numberlike=equation]{proposition}
\declaretheorem[name=Proposition,numbered=no]{proposition*}
\declaretheorem[numberlike=equation,style=noproofstyle,name=Proposition]{propositionwp}

\declaretheorem[numberlike=equation]{claim}
\declaretheorem[name=Claim,numbered=no]{claim*}
\declaretheorem[numberlike=equation,style=noproofstyle,name=Claim]{claimwp}

\declaretheorem[numberlike=equation]{conjecture}
\declaretheorem[name=Conjecture,numbered=no]{conjecture*}

\declaretheorem[numberlike=equation]{question}
\declaretheorem[name=Question,numbered=no]{question*}

\declaretheorem[name=Open Problem]{openproblem}
\declaretheorem[name=Exercise]{exercise}

\declaretheoremstyle[bodyfont=\it]{defstyle} 

\declaretheorem[numberlike=equation,style=defstyle]{definition}
\declaretheorem[unnumbered,name=Definition,style=defstyle]{definition*}

\declaretheorem[numberlike=equation,style=defstyle]{example}
\declaretheorem[unnumbered,name=Example,style=defstyle]{example*}

\declaretheorem[numberlike=equation,style=defstyle]{notation}
\declaretheorem[unnumbered,name=Notation=defstyle]{notation*}

\declaretheorem[numberlike=equation,style=defstyle]{construction}
\declaretheorem[unnumbered,name=Construction,style=defstyle]{construction*}

\declaretheoremstyle[]{rmkstyle} 

\newtheorem*{remark}{Remark}

\renewcommand{\subsubsectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}
\renewcommand{\sectionautorefname}{Section}
\newcommand{\algorithmautorefname}{Algorithm}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> garbage.tex <==

%%%%%%%%%%%
% GARBAGE %
%%%%%%%%%%%
\section{Garbage: $\sum_{i=2}^n\bw_{t,i}^2$}
We use $\Phi_t=\sum_{i=2}^n\bw_{t,i}^2$ as the potential function at time $t$. Observe that

\begin{align*}
\Exp\left[\Phi_{t+1}\ |\ \mathcal{F}_t\right] &= \Exp\left[\sum_{i=2}^n\bw_{t,i}^2+2\beta_t\Delta_{t,i}\bw_{t,i}+\beta_t^2\Delta_{t,i}^2\ |\ \mathcal{F}_t\right]\\
&\leq \Phi_t + 2\beta_t\cdot\left[\sum_{i=2}^n\left(\lambda_i-\sum_{j=1}^n\lambda_j\bw_{t,j}^2\right)\bw_{t,i}^2\right] + 4\beta_t^2\\
&= \Phi_t + 2\beta_t\cdot\left[\sum_{j=1}^n\lambda_j\bw_{t,j}^2 - \lambda_1\bw_{t,1}^2-\sum_{j=1}^n\lambda_j\bw_{t,j}^2\cdot\left(\|\bw_t\|_2^2-\bw_{t,1}^2\right)\right]+4\beta_t^2,
\intertext{By rearranging the terms, we have}
&= \Phi_t + 2\beta_t\cdot\left[\sum_{j=1}^n\lambda_j\bw_{t,j}^2\cdot\left(1-\|\bw_t\|_2^2\right)+\left(\sum_{j=1}^n\lambda_j\bw_{t,j}^2-\lambda_1\right)\cdot\bw_{t,1}^2\right] + 4\beta_t^2\\
(\because\autoref{lem:oja ub})&\leq \Phi_t + 2\beta_t\cdot\left[\gamma\cdot\sum_{j=1}^n\lambda_j\bw_{t,j}^2+\left(\sum_{j=1}^n\lambda_j\bw_{t,j}^2-\lambda_1\right)\cdot\bw_{t,1}^2\right] + 4\beta_t^2 \, .
\end{align*}
Let us zoom into the second term of the last inequality.
\begin{align*}
\gamma\cdot\sum_{j=1}^n\lambda_j\bw_{t,j}^2+\left(\sum_{j=1}^n\lambda_j\bw_{t,j}^2-\lambda_1\right)\cdot\bw_{t,1}^2 &\leq\gamma\lambda_2\Phi_t + \gamma\lambda_1\bw_{t,1}^2+\left(\lambda_2\Phi_t+\lambda_1\bw_{t,1}^2-\lambda_1\right)\cdot\bw_{t,1}^2\\
&=(1+\gamma)\lambda_2\Phi_t-(1-\gamma)\lambda_1\bw_{t,1}^2+\lambda_1(\|\bw_t\|_2^2-\Phi_t)\cdot\bw_{t,1}^2
\end{align*}




\section{Garbage: $\bw_{t,1}^2$}
\begin{theorem}\label{thm:oja w1 square weak}
For any $\epsilon,\delta\in(0,1)$, if $0\leq\beta_t\leq\min\{\frac{\epsilon\delta(\lambda_1-\lambda_2)}{16(\lambda_1+\lambda_2)},\frac{\lambda_2}{8\lambda_1(\lambda_1-\lambda_2)}\}$ for all $t\in\N$, and $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some monotonically increasing function $f$, then when $t\geq f^{-1}\left(\frac{\ln n(\lambda_1+\lambda_1)}{\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}\right)$, we have $\Pr\left[\bw_{t,1}^2<1-\epsilon\right]\leq\delta$.
\end{theorem}


\begin{table}[h]\label{table:oja w1 square weak}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
$\{\beta_t\}_{t\in\N}$                    & $f(t)$  & $f^{-1}(T)$                     & Convergence rate \\ \hline
$\beta_t=\frac{c_1}{(c_0+t)}$                     & $c_1\ln\left(\frac{t}{c_0}\right)$    & $c_0\exp(\frac{T}{c_1})$                 & $c_0\exp\left(\frac{\ln n(\lambda_1+\lambda_2)}{c_1\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}\right)$  \\ \hline
$\beta_t=c_1(c_0+t)^{\alpha-1}$, $\alpha\in(0,1)$ & $\frac{c_1}{\alpha}\left(t^{\alpha}-c_0^\alpha\right)$ &  $\left(\frac{\alpha T}{c_1}+c_0^\alpha\right)^{1/\alpha}$   & $\left(\frac{\alpha \ln n(\lambda_1+\lambda_2)}{c_1\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}+c_0^\alpha\right)^{1/\alpha}$    \\ \hline
$\beta_t=c$                               & $ct$        &       $\frac{T}{c}$          & $\frac{\ln n(\lambda_1+\lambda_2)}{c\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}$  \\ \hline
\end{tabular}
\caption{Convergence rate of Oja's rule from~\autoref{thm:oja w1 square weak} for different choices of $\{\beta_t\}_{t\in\N}$.}
\end{table}



In the following, we are going to use $\bw_{t,1}^2$ as the potential function and show that when $t$ is sufficiently large, the expectation of $\bw_{t,1}^2$ will be close to $1$. Thus, combining with~\autoref{lem:oja w norm ub}, we know that $\bw_{t,1}^2$ is close to $1$ with good probability.


For any $t\in\N$, consider the expectation of the square of the $(t+1)^{\text{th}}$ update, \textit{i.e.,} $\bw_{t+1,1}=\bw_{t,1}+\beta_t\Delta_{t,1}$, as follows.
\begin{equation}\label{eq:oja w1 square exp 1}
\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] = \bw_{t,1}^2 + 2\beta_t\cdot\left(\lambda_1-\sum_{i=1}^n\lambda_i\bw_{t,i}^2\right)\cdot\bw_{t,1}^2 + O(\beta_t^2) \, .
\end{equation}
The last term is actually within $[0,4\beta_t^2]$ due to the fact that $\Exp\left[\|\Delta_{t}\|_2^2\ |\ \mathcal{F}_t\right]\leq 4$. Now, rearrange the second term of~\autoref{eq:oja w1 square exp 1}, we have
\begin{align}
\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] &= \bw_{t,1}^2 + 2\beta_t\cdot\left[\lambda_1\bw_{t,1}^2-\lambda_1\bw_{t,1}^4 - \sum_{i=2}^n\lambda_i\bw_{t,i}^2\bw_{t,1}^2\right] + O(\beta_t^2)\nonumber\\
&\geq \bw_{t,1}^2 + 2\beta_t\cdot\left[\lambda_1\bw_{t,1}^2-\lambda_1\bw_{t,1}^4 - \lambda_2(\|\bw_t\|_2^2-\bw_{t,1}^2)\bw_{t,1}^2\right] + O(\beta_t^2)\nonumber\\
&\geq \bw_{t,1}^2 + 2\beta_t\cdot\left[\left(\lambda_1-(1+\gamma)\lambda_2\right)\bw_{t,1}^2-(\lambda_1-\lambda_2)\bw_{t,i}^4\right] + O(\beta_t^2) \, .\label{eq:oja w1 square exp 2}
\end{align}
The last inequality uses~\autoref{lem:oja w norm ub} to guarantee that $\|\bw_t\|_2^2\leq1+\gamma$.


\begin{lemma}\label{lem:oja w1 square exp}
For any $\epsilon\in(0,1)$, if $0\leq\beta_t\leq\min\{\frac{\epsilon(\lambda_1-\lambda_2)}{32\lambda_2},\frac{\lambda_2}{8\lambda_1(\lambda_1-\lambda_2)}\}$ for all $t\in\N$, and $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some monotonically increasing function $f$, then when $t\geq f^{-1}\left(\frac{2\ln n}{\epsilon(\lambda_1-\lambda_2)}\right)$, we have $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$.
\end{lemma}

\begin{proof}[Proof of~\autoref{lem:oja w1 square exp}]

\begin{claim}\label{claim:oja w1 square sink}
For any $t\in\N$ and $\epsilon\geq2\beta_t(\lambda_1-\lambda_2)(1+\gamma)^2$. If $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$, then $\Exp\left[\bw_{t+1,1}^2\right]\geq1-2\epsilon$.
\end{claim}
\begin{proof}[Proof of~\autoref{claim:oja w1 square sink}]
First, observe that $\Exp\left[\bw_{t,1}^4\right]=\Var\left[\bw_{t,1}^2\right]+\Exp\left[\bw_{t,1}^2\right]^2\geq(1-\epsilon)^2$.
Note that
\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right] &= \Exp\left[\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_{t}\right]\right]\\
(\autoref{eq:oja w1 square exp 2})&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t\cdot\left[\left(\lambda_1-(1+\gamma)\lambda_2\right)\bw_{t,1}^2-2\beta_t(\lambda_1-\lambda_2)\bw_{t,i}^4\right] + O(\beta_t^2)\right]\\
&\geq\Exp\left[\bw_{t,1}^2\right] - 2\beta_t(\lambda_1-\lambda_2)(1+\gamma)^2 \, .
\end{align*}
By the choice of $\epsilon$, $\gamma$, and $\beta_t$ (s.t. {\color{red} $\epsilon\geq2\beta_t(\lambda_1-\lambda_2)(1+\gamma)^2$}), we have $\Exp\left[\bw_{t+1,1}^2\right]\geq1-2\epsilon$.
\end{proof}

\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right] &= \Exp\left[\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_{t}\right]\right]\\
(\autoref{eq:oja w1 square exp 2})&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t\cdot\left[\left(\lambda_1-(1+\gamma)\lambda_2\right)\bw_{t,1}^2-2\beta_t(\lambda_1-\lambda_2)\bw_{t,i}^4\right]\right]\\
&=\int_{w=0}^{\sqrt{1+\gamma}}\left[\left(1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2\right)\right)\cdot w^2-(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]
\end{align*}
First,
\begin{align*}
&\int_{w=0}^{\sqrt{1-\epsilon}}\left[\left(1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2\right)\right)\cdot w^2-2\beta_t(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\\
\geq&\int_{w=0}^{\sqrt{1-\epsilon}}\left[1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2-(1-\epsilon)(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right] \\
=&\int_{w=0}^{\sqrt{1-\epsilon}}\left[1+2\beta_t\left(\frac{\epsilon}{2}(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right] \, .
\end{align*}
Next,
\begin{align}
&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[\left(1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2\right)\right)\cdot w^2-2\beta_t(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\nonumber\\
=&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2-(1-\epsilon)(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\nonumber\\
+&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}2\beta_t\left[(1-\epsilon)(\lambda_1-\lambda_2)w^2-(\lambda_1-\lambda_2)\cdot w^4\right]\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\label{eq:oja w1 square int 1}
\end{align}
Suppose $\Exp\left[\bw_{t,1}^2\right]\leq\tau$, then $\Pr\left[\bw_{t,1}^2\geq1-\epsilon\right]\leq\frac{\tau}{1-\epsilon}$.
\begin{align*}
\autoref{eq:oja w1 square int 1}\geq&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[1+2\beta_t\left(\lambda_1-(1+\gamma)\lambda_2-(1-\epsilon)(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\\
+&2\beta_t\left[(1-\epsilon)(\lambda_1-\lambda_2)(1+\gamma)-(\lambda_1-\lambda_2)(1+\gamma)^2\right]\cdot\tau\\
=&\int_{w=\sqrt{1-\epsilon}}^{\sqrt{1+\gamma}}\left[1+2\beta_t\left(\frac{\epsilon}{2}(\lambda_1-\lambda_2)\right)\right]\cdot w^2\cdot\Pr\left[\bw_{t,1}^2=w^2\right]\\
-&2\beta_t\tau(\lambda_1-\lambda_2)(1+\gamma)(\epsilon+\gamma) \, .
\end{align*}
Combine the two we have
\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right]&\geq \left[1+2\beta_t\left(\frac{\epsilon}{2}(\lambda_1-\lambda_2)\right)\right]\cdot \Exp\left[\bw_{t,1}^2\right] - 2\beta_t\tau(\lambda_1-\lambda_2)(1+\gamma)(\epsilon+\gamma) \, .
\end{align*}



---

Let us start with some observation on the expectation of the updates.

\vspace{2mm}
\noindent\textbf{Phase 1 ($\Exp\left[\bw_{t,1}^2\right]<1-\epsilon$).}
In this case, we are going to show that the expectation of $\bw_{t+1,1}^2$ increases by a non-negligible amount of growth.
\begin{align*}
\Exp\left[\bw_{t+1,1}^2\right] &=\Exp\left[\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right]\right]\\
(\autoref{eq:oja w1 square exp 2})&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t(\lambda_1-(1+\gamma)\lambda_2)\bw_{t,1}^2-(\lambda_1-\lambda_2)\bw_{t,1}^4 + O(\beta_t^2)\right]\\
()&\geq \Exp\left[\bw_{t,1}^2 + 2\beta_t\left[(\lambda_1-(1+\gamma)\lambda_2)-(\lambda_1-\lambda_2)\right]\bw_{t,1}^2 + O(\beta_t^2)\right]\\
&\geq \bw_{t,1}^2 + \epsilon\beta_t(\lambda_1-\lambda_2)\bw_{t,1}^2
\end{align*}
where the last inequality is due to the choice of $\gamma$ ({\color{red} $\gamma\leq\frac{\epsilon(\lambda_1-\lambda_2)}{2\lambda_2}$}) such that $\lambda_1-(1+\gamma)\lambda_2\geq(1-\epsilon/2)(\lambda_1-\lambda_2)$.

\vspace{2mm}
\noindent\textbf{Phase 2 ($1-\epsilon\leq\bw_{t,1}^2$).}
In this case, we are going to show that the expectation of $\bw_{t+1,t}^2$ is still larger than $1-\epsilon$. Consider two cases: (i) $1-\epsilon\leq\bw_{t,1}^2\leq1-\epsilon/2$ and (ii) $1-\epsilon/2\leq\bw_{t,1}^2\leq1+\gamma$. For case (i), using the same argument in Phase 1, one can see that $\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] \geq \bw_{t,1}^2\geq1-\epsilon$.
For case (ii), we have
\begin{align}
\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] &\geq \bw_{t,1}^2 + 2\beta_t\left[(1-\epsilon/2)(\lambda_1-\lambda_2)\bw_{t,1}^2-(\lambda_1-\lambda_2)\bw_{t,1}^4\right] + O(\beta_t^2)\nonumber\\
&\geq \bw_{t,1}^2 + 2\beta_t(\lambda_1-\lambda_2)(1+\gamma)\left[(1-\epsilon/2)-(1+\gamma)\right]\nonumber\\
&\geq\bw_{t,1}^2 -2\beta_t(\lambda_1-\lambda_2)(1+\gamma)(\epsilon/2+\gamma) \, .\label{eq:oja w1 square phase 2}
\end{align}
By the choice of $\beta_t$ ({\color{red} $\beta_t\leq\frac{\epsilon}{4(\lambda_1-\lambda_2)(1+\gamma)(\epsilon/2+\gamma)}$}), the last term in the last inequality is at least $-\epsilon/2$ and thus we still have $\Exp\left[\bw_{t+1,1}^2\ |\ \mathcal{F}_t\right] \geq \bw_{t,1}^2-\epsilon/2\geq1-\epsilon$.


Now, we are ready to show that when $t\geq f^{-1}\left(\frac{2\ln n}{\epsilon(\lambda_1-\lambda_2)}\right)$, $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$. First, let us rewrite $\Exp\left[\bw_{t,1}^2\right]$ using the filtration for $\{\bw_t\}_{t\in\N}$ as follows.
$$
\Exp\left[\bw_{t,1}^2\right] = \Exp\left[\Exp\left[\cdots\Exp\left[\bw_{t,1}^2\ |\ \mathcal{F}_{t-1}\right]\cdots\right]\ |\ \mathcal{F}_0\right] \, .
$$
For the sake of contradiction, suppose $\Exp\left[\bw_{t,1}^2\right]<1-\epsilon$. By the above discussion, for each $t'=1,2,\dots,t-1$, we have
$$
\Exp\left[\bw_{t'+1,1}^2\ |\ \mathcal{F}_{t'}\right]\geq(1+\epsilon\beta_t(\lambda_1-\lambda_2))\cdot\bw_{t',1}^2 \, .
$$
By the choice of $\beta_{t'}$ ({\color{red} $\beta_{t'}\leq\frac{1}{2\epsilon(\lambda_1-\lambda_2)}$}), we have $(1+\epsilon\beta_{t'}(\lambda_1-\lambda_2))\geq\exp(\epsilon\beta_t(\lambda_1-\lambda_2))$ for each $t'\in\N$.
Thus,
\begin{align*}
\Exp\left[\bw_{t,1}^2\right] &\geq \prod_{t'=0}^{t-1}(1+\epsilon\beta_{t'}(\lambda_1-\lambda_2))\cdot \bw_{0,1}^2\\
&\geq \exp\left(\frac{\epsilon(\lambda_1-\lambda_2)}{2}\sum_{t'=0}^{t-1}\beta_{t'}\right)\cdot\frac{1}{n}\\
&\geq1-\epsilon
\end{align*}
which is a contradiction. Thus, we conclude that $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon$.
\end{proof}



\begin{proof}[Proof of~\autoref{thm:oja w1 square weak}]
Pick $\epsilon'=\frac{2\epsilon\delta\lambda_2}{\lambda_1+\lambda_2}$ and $\gamma=\frac{\epsilon'(\lambda_1-\lambda_2)}{2\lambda_2}$ such that $\frac{\epsilon'+\gamma}{\epsilon+\gamma}\leq\delta$. Apply~\autoref{lem:oja w1 square exp} using $\epsilon'$, when $t\geq f^{-1}\left(\frac{\ln n(\lambda_1+\lambda_1)}{\epsilon\delta\lambda_2(\lambda_1-\lambda_2)}\right)=f^{-1}\left(\frac{2\ln n}{\epsilon'(\lambda_1-\lambda_2)}\right)$, we have $\Exp\left[\bw_{t,1}^2\right]\geq1-\epsilon'$. Next, by~\autoref{lem:oja w norm ub}, we can upper bound the expectation as follows. Let $p=\Pr\left[\bw_{t,1}^2<1-\epsilon\right]$, we have
$$
\Exp\left[\bw_{t,1}^2\right]\leq (1-\epsilon)p+(1+\gamma)(1-p) = 1+\gamma-(\epsilon+\gamma)p
$$
and thus
$$
p\leq\frac{\epsilon'+\gamma}{\epsilon+\gamma}\leq\delta.
$$
\end{proof}



%%%%%%%%%%%
% Garbage %
%%%%%%%%%%%
\section{Garbage: Log ratio}
\begin{theorem}\label{thm:oja Chebyshev}
For any $\epsilon,\delta\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some function $f$ where $\lim_{t\rightarrow\infty}f(t)=\infty$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then when $t\geq \max\{f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{\lambda_1-\lambda_2}\right),f^{-1}\left(\frac{\sqrt{O(1)/\delta}+\frac{1}{2}\ln n+O(1)}{\lambda_1-\lambda_2}\right)\}$, with probability $1-\delta$, we have
$$
\frac{\bw_{t,1}^2}{\|\bw_t\|_2^2}\geq1-\epsilon \, .
$$
\end{theorem}

\iffalse
\begin{theorem}\label{thm:oja Chebyshev}
For any $\epsilon,\delta\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq\alpha\cdot\ln t$ for large enough $t$ and some $\alpha>0$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then when $t\geq e^{\max\{\frac{\ln(n/\epsilon^2)+O(1)}{\alpha(\lambda_1-\lambda_2)},O(\frac{\ln(n)}{\sqrt{\delta}\alpha(\lambda_1-\lambda_2)})\}}$, with probability $1-\delta$, we have
$$
\frac{\bw_{t,1}^2}{\|\bw_t\|_2^2}\geq1-\epsilon \, .
$$
\end{theorem}
\fi

Here we state~\autoref{thm:oja Chebyshev} in a very general form with the flexibility to choose different $\{\beta_t\}_{t\in\N}$. A standard choice would be $\beta_t=\frac{c}{t}$ for some constant $c>0$ and the corresponding $f$ would be $f(t)\geq c\ln t$. In~\autoref{table:oja Chebyshev}, we list the convergence rate bounds for different choices of $\{\beta_t\}_{t\in\N}$.

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline
$\{\beta_t\}_{t\in\N}$                      & $f(t)$                       & Convergence rate                                                                                                                                                            \\ \hline
$\beta_t=\frac{c}{t}$                       & $c\ln t$                     & $t\geq\max\{ e^{\frac{\ln(n/\epsilon^2)+O(1)}{c(\lambda_1-\lambda_2)}},e^{O(\frac{\ln(n)}{\sqrt{\delta}c(\lambda_1-\lambda_2)})}\}$                                             \\ \hline
$\beta_t=ct^{\alpha-1}$, $\alpha\in(0,0.5)$ & $\frac{c}{\alpha}t^{\alpha}$ & $t\geq \max\{\left(\frac{\alpha\left(\ln(1/\epsilon)+O(1)\right)}{c(\lambda_1-\lambda_2)}\right)^{1/\alpha},\left(\frac{\alpha\left(\sqrt{O(1)/\delta}+\frac{1}{2}\ln n+O(1)\right)}{c\left(\lambda_1-\lambda_2\right)}\right)^{1/\alpha}\}$ \\ \hline
\end{tabular}
\caption{Convergence rate for different choices of $\{\beta_t\}_{t\in\N}$.}
\label{table:oja Chebyshev}
\end{table}

The proof of~\autoref{thm:oja Chebyshev} is based on the following three lemmas and Chebyshev's inequality. The first lemma shows that by properly picking $\{\beta_t\}_t$, the $\ell_2$ norm of $\bw_t$ is always close to $1$.
\begin{lemma}\label{lem:oja ub}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{\epsilon}{16}$ for all $t\in\N$, then $1-\epsilon\leq\|\bw_t\|_2^2\leq 1+\epsilon$ for all $t\in\N$.
\end{lemma}
\begin{proof}
Here we only prove the upper bound while the lower bound can be proved using the same argument.
The proof is using induction. For $t=0$, we have $\|\bw_0\|_2=1$ from the setting. For each $t\geq0$, we have
\begin{align*}
\|\bw_t+1\|_2^2 &= \|\bw_t\|_2^2 + 2\beta_t\cdot\bw_t^\top\left[\bx_t^\top\bw_t\bx_t-(\bx_t^\top\bw_t)^2\bw_t\right] + \beta_t^2\cdot\|\bx_t^\top\bw_t\bx_t-(\bx_t^\top\bw_t)^2\bw_t\|^2\\
&=\|\bw_t\|_2^2 - 2\beta_t(\bx_t^\top\bw_t)^2\cdot(\|\bw_t\|_2^2-1) + 4\beta_t^2(\bx_t^\top\bw_t)^2\cdot\max\{\|\bx_t\|_2^2,(\bx_t^\top\bw_t)^2\|\bw_t\|_2^2\} \, .
\end{align*}
Finally, consider two cases: (i) $\|\bw_t\|_2^2\leq1+\epsilon/2$ and (ii) $1+\epsilon/2<\|\bw_t\|_2^2\leq1+\epsilon$. It is then not difficult to see that by our choice of $\beta_t$, we have $\|\bw_{t+1}\|_2^2\leq1+\epsilon$ in both cases. This completes the induction and the proof.
\end{proof}

Note that~\autoref{lem:oja ub} does not depend on the structure of $A$ and holds with probability $1$.

The other two lemmas describe the expectation and the variance of the log of the ration between the $\ell_2$ mass of the first coordinate and that of the rest. However, it turns out that directly working on the log of the ratio would not work due to the unbounded second moment. As a fix, we are going to work on the \textit{truncated} version of the log ratio and show that the original log ratio behaves the same as its truncated counterpart in most of the time. To formalize the above idea, we are going to use the language from martingale theory. See~\autoref{sec:prelim} for basic definitions of martingale. 

Fix $t\in\N$ and for each $t'\in\{0,1,\dots,t\}$, let
$$
M_{t'} = \Exp\left[\sum_{i=2}^n\bw_{t,i}^2\Big|\mathcal{F}_{t'}\right] \, .
$$
It is not difficult to check that $\{M_{t'}\}_{t'\in\{0,1,\dots,t\}}$ is a martingale.
Also, observe that $M_0=\Exp\left[\sum_{i=2}^n\bw_{t,i}^2\right]$ and $M_t=\sum_{i=2}^n\bw_{t,i}^2$. Namely, $|M_t-M_0|$ is exactly the deviation of the $\ell_2$ mass to its expectation.



The second key lemma upper bounds the log of the ratio between the $\ell_2$ mass of the first coordinate and that of the rest.
\begin{lemma}\label{lem:oja ratio}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ for some function $f$ where $\lim_{t\rightarrow\infty}f(t)=\infty$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq\ln\left(\frac{1}{\epsilon}\cdot\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)$ when $t\geq f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{2(\lambda_1-\lambda_2)}\right)$.
\end{lemma}

\iffalse
\begin{lemma}\label{lem:oja ratio}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq\alpha\cdot\ln t$ for large enough $t$ and some $\alpha>0$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq\ln\left(\frac{1}{\epsilon}\cdot\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)$ when $t\geq e^{\frac{\ln(1/\epsilon)+O(1)}{\alpha(\lambda_1-\lambda_2)}}$.
\end{lemma}
\fi

Finally, we need the following lemma upper bounding the variance of the log ratio.
\begin{lemma}\label{lem:oja ratio variance}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$ and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $\Var\left[\sum_{i=2}^n\bw_{t,i}^2\right]=O(1)$ for all $t\in\N$.
\end{lemma}

Before we prove~\autoref{lem:oja ratio} and~\autoref{lem:oja ratio variance}, let us see how the above lemmas combining with Chebyshev's inequality imply the main theorem.
\begin{proof}[Proof of~\autoref{thm:oja Chebyshev}]
By Chebyshev's inequality, we have
$$
\Pr\left[\left|\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)-\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\right|>\sqrt{\frac{\Var[X_t]}{\delta}}\right]\leq\delta \, .
$$
Next, recall that $\bw_{0,i}^2=\frac{1}{n}$ for each $i\in[n]$ and thus by the choice of $t\geq \max\{f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{\lambda_1-\lambda_2}\right),f^{-1}\left(\frac{\sqrt{O(1)/\delta}+\frac{1}{2}\ln n+O(1)}{\lambda_1-\lambda_2}\right)\}$, \autoref{lem:oja ratio} and~\autoref{lem:oja ratio variance} give us that
$$
\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq2\ln\left(\frac{1}{\epsilon}\right),\ 2\sqrt{\frac{\Var[X_t]}{\delta}}
$$
Finally,
$$
\Pr\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)<\ln\left(\frac{1}{\epsilon}\right)\right]\leq\delta \, .
$$
\end{proof}

\subsection{Details of the expectation bound}
\begin{proof}[Proof of~\autoref{lem:oja ratio}]
Note that one can expand the expectation $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]$ using the filtration of the process $\bw_t$. Concretely, we have
\begin{equation}\label{eq:oja exp filtration}
\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right] = \Exp\left[\Exp\left[\cdots\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\Big|\ \bw_{t-1}\right]\cdots\right]\Big|\ \bw_{1}\right] \, .
\end{equation}
Now, it suffices to prove the following claim.
\begin{claim}\label{claim:oja ratio induction step}
For any $t\in\N$, we have
$$
\Exp\left[\ln\left(\bw_{t,1}^2\right)\Big|\ \bw_{t-1}\right]=\ln\left(\bw_{t-1,1}^2\right) + 2\beta_{t-1}\cdot\left(\lambda_1-\sum_{i'\in[n]}\lambda_i\bw_{t-1,i'}^2\right) + \Theta(\beta_{t-1}^2)
$$
and
$$
\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\Big|\ \bw_{t-1}\right]=\ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + 2\beta_{t-1}\cdot\left(\frac{\sum_{i=2}^n\lambda_i\bw_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right) + \Theta(\beta_{t-1}^2) \, .
$$
\end{claim}
\begin{proof}[Proof of~\autoref{claim:oja ratio induction step}]
For brevity, here we only prove the second equation while the first equation can be proved in similar argument.
By~\autoref{eq:oja}, let $\Delta_{t-1,t}=\left(y_t(\bx_t-y_t\bw_t)\right)_i$, we have
\begin{align*}
\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\Big|\ \bw_{t-1}\right] &=\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t-1,i}^2 + 2\beta_{t-1}\Delta_{t-1,i}\bw_{t-1,i} + \beta_{t-1}^2\Delta_{t-1,i}^2\right)\Big|\ \bw_{t-1}\right]\\
&= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + \Exp\left[\ln\left(1+2\beta_{t-1}\frac{\sum_{i=2}^n\Delta_{t-1,i}\bw_{t-1,i}}{\sum_{i=2}^n\bw_{t-1,i}^2} + \beta_{t-1}^2\frac{\sum_{i=2}^n\Delta_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}\right)\Big|\ \bw_{t-1}\right]\\
&= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + \Exp\left[2\beta_{t-1}\frac{\sum_{i=2}^n\Delta_{t-1,i}\bw_{t-1,i}}{\sum_{i=2}^n\bw_{t-1,i}^2} + \Theta\left(\beta_{t-1}^2\frac{\sum_{i=2}^n\Delta_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}\right)\Big|\ \bw_{t-1}\right]
\end{align*}
By~\autoref{eq:oja exp}, for each $i\in[n]$, we have 
$$
\Exp\left[\Delta_{t-1,i}\Big|\ \bw_{t-1}\right]=\left(\lambda_i-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right)\bw_{t-1,i}
$$
and thus combining with~\autoref{lem:oja ub}, we have\todo{Here I'm a bit sloppy about the $\beta_{t-1}^2$ term}
\begin{align*}
\Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\Big|\ \bw_{t-1}\right] &= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + 2\beta_{t-1}\cdot\frac{\sum_{i=2}^n\left(\lambda_i-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right)\cdot\bw_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2} + \Theta(\beta_{t-1}^2)\\
&= \ln\left(\sum_{i=2}^n\bw_{t-1,i}^2\right) + 2\beta_{t-1}\cdot\left(\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t-1,i}^2}{\sum_{i=2}^n\bw_{t-1,i}^2}-\sum_{i'\in[n]}\lambda_{i'}\bw_{t-1,i'}^2\right) + \Theta(\beta_{t-1}^2) \, .
\end{align*}
\end{proof}
By applying~\autoref{claim:oja ratio induction step} on~\autoref{eq:oja exp filtration}, we have
\begin{align*}
\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right] &= \Exp\left[\ln\left(\bw_{t,1}^2\right)\right] - \Exp\left[\ln\left(\sum_{i=2}^n\bw_{t,i}^2\right)\right]\\
&=\ln\left(\bw_{0,1}^2\right) - \ln\left(\sum_{i=2}^n\bw_{0,i}^2\right)+2\sum_{t'=0}^{t-1}\beta_{t'}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) + \Theta\left(\sum_{t'=0}^{t-1}\beta_{t'}^2\right)\\
&\geq\ln\left(\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)+2(\lambda_1-\lambda_2)\cdot f(t) - O(1)\, .
\end{align*}
Note that the last inequality is due to the choice of $\{\beta_t\}_t$ where $\sum_{t'=0}^{t-1}\beta_{t'}\geq f(t)$ and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$.
Finally, by our choice of $t\geq f^{-1}\left(\frac{\ln(1/\epsilon)+O(1)}{2(\lambda_1-\lambda_2)}\right)$, we conclude that $\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]\geq\ln\left(\frac{1}{\epsilon}\cdot\frac{\bw_{0,1}^2}{\sum_{i=2}^n\bw_{0,i}^2}\right)$.
\end{proof}

\subsection{Details of the variance bound}
\todo{Maybe need some prelim for conditional variance and filtration.}

Now, we are ready to prove~\autoref{lem:oja ratio variance} with the aid of~\autoref{lem:var decomp}.

\begin{proof}[Proof of~\autoref{lem:oja ratio variance}]
For each $t\in\N$, let $X_t=\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)$ and apply~\autoref{lem:var decomp}. The key step of the proof is showing that each summand in the variance decomposition is nicely upper bounded.
\begin{claim}\label{claim:oja ratio variance bound}
For each $t'\in\N$, we have
$$
\Exp\left[\Var\left[\Exp\left[X_t|\mathcal{F}_{t'+1}\right]|\mathcal{F}_{t'}\right]\right] = O(\beta_{t'}^2) \, .
$$
\end{claim}
Note that as $\sum_{t'=0}^\infty\beta_{t'}=O(1)$,~\autoref{claim:oja ratio variance bound} combining with~\autoref{lem:var decomp} immediately give that $\Var\left[X_t\right]=O(1)$. Now, the only thing left is proving~\autoref{claim:oja ratio variance bound}.
\begin{proof}[Proof of~\autoref{claim:oja ratio variance bound}]
Recall that from the definition of conditional variance we have
$$
\Var\left[\Exp\left[X_t|\mathcal{F}_{t'+1}\right]|\mathcal{F}_{t'}\right] = \Exp\left[\left(\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right]\right)^2\right] \, .
$$
By~\autoref{claim:oja ratio induction step}, we have
\begin{align}
\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right] &= \ln\left(\frac{\bw_{t'+1,1}^2}{\sum_{i=2}^n\bw_{t'+1,i}^2}\right) + 2\sum_{t''=t'+1}^{t-1}\beta_{t''}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t'',i}^2}{\sum_{i=2}^n\bw_{t'',i}^2}\right) + \Theta(\beta_{t''}^2)\nonumber\\
&- \left(\ln\left(\frac{\bw_{t',1}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) + 2\sum_{t''=t'}^{t-1}\beta_{t''}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t'',i}^2}{\sum_{i=2}^n\bw_{t'',i}^2}\right) + \Theta(\beta_{t''}^2)\right)\nonumber\\
&= \ln\left(\frac{\bw_{t'+1,1}^2}{\sum_{i=2}^n\bw_{t'+1,i}^2}\right) - \ln\left(\frac{\bw_{t',1}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) - 2\beta_{t'}\cdot\left(\lambda_1-\frac{\sum_{i=2}^n\lambda_i\cdot\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) + \Theta(\beta_{t'}^2) \, .\label{eq:oja ratio variance 1}
\end{align}
Recall that $\bw_{t'+1,i}=\bw_{t',i}+\beta_{t'}\cdot\Delta_{t',i}$, thus we have\todo{I'm a bit fast here, can slow down if needed.}
\begin{align}
\ln\left(\frac{\bw_{t'+1,1}^2}{\sum_{i=2}^n\bw_{t'+1,i}^2}\right) - \ln\left(\frac{\bw_{t',1}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right) &= 2\beta_{t'}\cdot\left(\frac{\Delta_{t',1}}{\bw_{t',1}}-\frac{\sum_{i=2}^n\Delta_{t',i}\bw_{t',i}}{\sum_{i=2}^n\bw_{t',i}^2}\right) + \Theta(\beta_{t'}^2) \, .\label{eq:oja ratio variacne 2}
\end{align}
Combining~\autoref{eq:oja ratio variance 1} and~\autoref{eq:oja ratio variacne 2} we have
\begin{align}
\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right] &=2\beta_{t-'}\cdot\left[\left(\frac{\Delta_{t',1}}{\bw_{t',1}}-\frac{\sum_{i=2}^n\Delta_{t',i}\bw_{t',i}}{\sum_{i=2}^n\bw_{t',i}^2}\right)-\left(\lambda_1-\frac{\sum_{i=2}^2\lambda_i\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right)\right] + \Theta(\beta_{t'}^2) \, .\label{eq:oja ratio variance 3}
\end{align}
Thus, combining with~\autoref{lem:oja ub} we have\todo{I'm a bit sloppy here. Basically we still need to argue that the expectation of the square of $\frac{\Delta_{t',1}}{\bw_{t',1}}$ is $O(1)$.}
$$
\Var\left[\Exp\left[X_t|\mathcal{F}_{t'+1}\right]|\mathcal{F}_{t'}\right] = \Exp\left[\left(\Exp\left[X_t|\mathcal{F}_{t'+1}\right]-\Exp\left[X_t|\mathcal{F}_{t'}\right]\right)^2\right] =O(\beta_{t'}^2)\, .
$$
\end{proof}
This completes the proof of~\autoref{lem:oja ratio variance}.
\end{proof}

\subsection{High probability bound}

To get high probability bound, \textit{i.e.,} having exponentially better dependency on error probability $\delta$, we are going to apply tools from martingale theory. Also, it is important to identify the right martingale to analyze the following is our choice. Fix $t\in\N$ and for each $t'\in\{0,1,\dots,t\}$, let
$$
M_{t'} = \Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\Big|\mathcal{F}_{t'}\right] \, .
$$
It is not difficult to check that $\{M_{t'}\}_{t'\in\{0,1,\dots,t\}}$ is a martingale.
Also, observe that $M_0=\Exp\left[\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)\right]$ and $M_t=\ln\left(\frac{\bw_{t,1}^2}{\sum_{i=2}^n\bw_{t,i}^2}\right)$. Namely, $|M_t-M_0|$ is exactly the deviation of the log ratio to its expectation. Finally, to apply concentration inequality for martingale (\textit{e.g.,} Azuma's inequality in~\autoref{lem:azuma}), it suffices to upper bound the absolute difference between $|M_{t'+1}-M_{t'}|$ for each $t'\in\{0,1,\dots,t-1\}$.

\begin{lemma}\label{lem:oja abs diff}
For any $\epsilon\in(0,1)$, if $\beta_t\leq\frac{1}{16\lambda_1}$ for all $t\in\N$, $\sum_{t'=0}^{t-1}\beta_{t'}\geq\alpha\cdot\ln t$ for large enough $t$ and some $\alpha>0$, and $\sum_{t'=0}^\infty\beta_{t'}^2=O(1)$, then $|M_{t'+1}-M_{t'}|=O(\beta_{t'})$ with probability $1$ for each $t'\in\{0,1,\dots,t-1\}$.
\end{lemma}
\begin{proof}[Proof of~\autoref{lem:oja abs diff}]
Note that using the notation from the previous lemmas, $M_{t'}=\Exp\left[X_t|\mathcal{F}_{t'}\right]$. Thus, by~\autoref{eq:oja ratio variance 3}, we have
\begin{align*}
M_{t'+1}-M_{t'} &= \Exp\left[X_t|\mathcal{F}_{t'+1}\right] - \Exp\left[X_t|\mathcal{F}_{t'}\right]\\
&= 2\beta_{t'}\cdot\left[\left(\frac{\Delta_{t',1}}{\bw_{t',1}}-\frac{\sum_{i=2}^n\Delta_{t',i}\bw_{t',i}}{\sum_{i=2}^n\bw_{t',i}^2}\right)-\left(\lambda_1-\frac{\sum_{i=2}^2\lambda_i\bw_{t',i}^2}{\sum_{i=2}^n\bw_{t',i}^2}\right)\right] + \Theta(\beta_{t'}^2)
\end{align*}
\end{proof}


